Extending the Interaction Nets Calculus by Generic Rules

We extend the textual calculus for interaction nets by generic rules and propose constraints to preserve uniform confluence. Furthermore, we discuss the implementation of generic rules in the language inets, which is based on the lightweight interaction nets calculus.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{S.Alves and I. Mackie (Eds.): Second International Workshop\\ on Linearity 2012 (LINEARITY'12).\\
EPTCS 101, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.101.2}{10.4204/EPTCS.101.2}}

